Interpretable Node Representation with Attribute Decoding

Variational Graph Autoencoders (VGAEs) are powerful models for unsupervised learning of node representations from graph data. In this work, we systematically analyze modeling node attributes in VGAEs and show that attribute decoding is important for node representation learning. We further propose a new learning model, interpretable NOde Representation with Attribute Decoding (NORAD). The model encodes node representations in an interpretable approach: node representations capture community structures in the graph and the relationship between communities and node attributes. We further propose a rectifying procedure to refine node representations of isolated notes, improving the quality of these nodes' representations. Our empirical results demonstrate the advantage of the proposed model when learning graph data in an interpretable approach.

==> figures/reconstruct_x_figure.tex <==

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.47\textwidth]{figures/dirt_attention.pdf}
    \end{center}
    \vspace*{-8pt}
    \caption{Neural Topic Attention: The Query(Q) is obtained from topic context vector transformed by MLP; Key(K) is mapped from word embedding by another MLP; u of each word is then calculated from Q and K.}
    \label{fig:attention}
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> response.tex <==
R5jC: 

Q1: It is not clear if the baselines have a number of parameters comparable to the proposed method. Does the extra performance come at a significant computational cost? If so, this should be quantified and discussed.
R1: For the encoder, since NORAD uses a shallower but wider GCN compared to the baselines, our encoder tends to contain more parameters compared to the baselines. However, we argue that most of the parameters can be pruned out as the learned sparse representations indicate that most of the network parameters are not effective. Appendix A.2 further provides the encoder configurations of the baselines and NORAD, which states that the parameters of the NORAD's encoder can be brought down without sacrificing the performance. On the other hand, the extra parameters of the decoder do not contribute to the computation. Because the decoders come with the purpose of providing better guidance of the encoding quality, and the examination of the quality of node representation only relies on the encoder. 

Q2: The experiments are conducted on very few and small datasets. The GNN community has long moved past the citation networks, so I advise the authors run their experiments on better datasets like OGB or similar. As it is, the results are unlikely to transfer to practical/non-benchmark problems.

Q3: The experiment on interpretability should also compare the interpretability of the other baselines. As it is, it is not clear if the proposed method is actually more interpretable than the baselines.
R3: 


In general, the interpretability of our model can be analyzed via the prior, the node decoder, and the block model. 

Because the prior adopted by most baselines do not shape the learned representations to enable interpretability. We only analyze the interpretability of the baselines by inspecting the shape of the embedding distribution. We provide the t-SNE visualizations for each baseline (See Figure 5 in Appendix) to illustrate that NORAD learns more separable embeddings compare to the baselines. 

typos: 

==> sections/variational_em.tex <==
\section{Variational EM for NTB}
In this section, we introduce the variational EM method to perform the inference and training for NTB. NTB models the joint probability of the observed variables $X$ and $A$, which can be trained by maximizing the log-likelihood. However, estimating the log-likelihood is computationally intractable as it involves marginalization in the continuous space. Instead, we maximize the evidence lower bound (ELBO) on $\log{p_\theta(X,A)}$. The ELBO $\mathcal{L}(\phi, \theta, A, X|B) \leq \log{p_\theta(X,A)}$ is
\begin{align}
    &\mathcal{L}(\phi, \theta, A, X|B) \label{elbo} \\
    &= \mathrm{E}_{q_\phi}\big[\log{p_\theta(A,X,C,Z,V|B) - \log{q_\phi(Z,V,C|A,X)}}\big] \nonumber
\end{align}
Here $q_\phi(Z,V,C|A,X)$ is a variational distribution to approximate the posterior $p_\theta(Z,V,C|X,A,B)$. We jointly optimize the model parameters $\theta$ and the variational parameters $\phi$ by maximizing \eqref{elbo}. We alternatively optimize $\theta, \phi$ and $B$ in a variational EM fashion. In E-step (sec \ref{Estep}), We consider block model $B$ as the hyperparameters when maximizing the ELBO (E-step). In M-step (sec \ref{Mstep}), we fix the parameters $\theta, \phi$ and optimize $B$ to maximize the log-likelihood. The intuition behind this is that we design and isolate the training of the block model to capture clear relations between different topics. We reparameterize the distribution of the random variables to make the objective function differentiable on them. Then we can train with Stochastic Gradient Variational Bayes (SGVB). The details are in Appendix (). The training procedure is shown in Algorithm \ref{alg:training_algorithm_graphrnn}.

\begin{algorithm}[t]
  \caption{Varaitional EM for Neural Topic Blockmodel}
  \label{alg:training_algorithm_graphrnn}
  \begin{algorithmic}
    \STATE {\bfseries Input:} Dataset of graph $G = (X,A)$, 
    \STATE {\bfseries Output:} Learned node-wise representation $r$ and Blockmodel $B$
    \REPEAT   
        \STATE Initialize $(B, \theta, \phi)$
        \FOR{E step $= 1, \cdots $}
            \STATE Fix Blockmodel $B$
            \STATE Sample $r \sim q_{\phi}(r|X, A)$
            \STATE Optimize ($\phi, \theta$) by maximizing $\mathcal{L}(\phi, \theta, A, X|B)$
        \ENDFOR
        \FOR{M step $= 1, \cdots $}
            \STATE Fix parameters ($\phi, \theta$)
            \STATE Optimize $B$ by maximizing $\mathcal{L}(\phi, \theta, A, X|B)$
        \ENDFOR
    \UNTIL{convergence of the ELBO $\mathcal{L}(\phi, \theta, A, X|B)$}
  \end{algorithmic}
\end{algorithm}
% \begin{align}
%     p(A,X) = \int_{V,\Pi}\sum_{Z}p(A,X,\Pi,Z,V|B,\mathbb{E}^t,\mathbb{E}^w)dVd\Pi
% \end{align}
% where we have the joint probability $p(A,X,C,Z,V)$, which can be factorized into:
% \begin{align}
%     &p(A,X,C,Z,V)\\
%     &=p(A|Z,V,B)p(X|Z,V,\mathbb{E}^t,\mathbb{E}^w)p(Z|\Pi)p(\Pi|a,b)p(V|\mu,\sigma)
% \end{align}

\subsection{E-step}
\label{Estep}
In the E-step, we compute the variational distribution of the latent variables given observations $q_\phi(Z,V,C|A,X)$ to approximate the true posterior $p_\theta(Z,V,C|A,X,B)$. Here we choose to use the mean-field approximation. The mean-field variational distribution assume each latent variable is independent
\begin{align}
    q_\phi(Z,V,C|A,X) = q_\phi(Z|A,X)q_\phi(V|A,X)q_\phi(C|A,X)
\end{align}
where $q_\phi(Z|A,X)$ follows the Bernoulli distribution, $q_\phi(V|A,X)$ follows the Gaussian distribution, and $q_\phi(C|A,X)$ follows the Beta distribution. Each node has its own variational parameters,
\begin{align}
    q_\phi(c_{nk}) &= \mathrm{Beta}(a_{nk},b_{nk}) \\
    q_\phi(z_{nk}) &= \mathrm{Bernoulli}(\pi_{nk}) \\
    q_\phi(v_{nk}) &= \mathcal{N}(\mu_{nk}, \sigma_{nk})\\
    \{a_{nk},b_{nk},\pi_{nk},\mu_{nk},& \sigma_{nk}\}^{N,K}_{n,k=1}=\mathrm{GNN}_\phi(X,A)
\end{align}
We consider Graph Neural Network (GNN) as the key component to approximate the variational parameters. Here we choose Graph Convolutional Network (GCN), which can be replaced by other networks (e.g. GraphSAGE). The use of GCN passes neighboring node topic messages through the link to better learn the latent node representation in the Graph.
\subsection{M-step}
\label{Mstep}
In the M-step, we maximize the log-likelihood of $\log{p(A,X|B)}$ with parameters $\{\theta, \phi\}$ fixed, and optimize block model $B$. Again since the estimation of log-likelihood is intractable, we instead optimize the ELBO via SGD. Because the only term with respect to $B$ is $p(A|B)$, we can disregard other terms and maximize
\begin{align}
\mathcal{L}(\phi^*, A,X,B) = \mathrm{E}_{q_{\phi}}\Big[\log{p(A|Z,C,V,B)}\Big] -\lambda ||B||_1 
\end{align}
here we introduce an L1 regularization term on the block model $B$, with coefficent $\lambda=0.001$. When topic $i$ and topic $j$ have strong relation with each other, the first term dominates and the entry $B_{ij}$ tends to have a meaningful value. Otherwise, the second term dominates and the entry $B_{ij}$ tends to be zero, providing no information.
% \subsection{Reparameterization}
% \label{Reparam}
% $v$ is sampled using reparameterization trick so that the Monte Carlo estimation of the normal distribution. $q(v)$ is differentiable:
% \begin{align}
%     v_{nk} = \mu_{nk} + \sigma_{nk} \epsilon,\; \epsilon \sim \mathcal{N}(0, 1)
% \end{align}

% We approximate the Beta distribution $q(c)$ with Kumaraswamy distribution:
% \begin{align}
%     u &\sim \mathrm{Uniform}(0,1) \\
%     c_{nk} &= (1 - u^{\frac{1}{b_{nk}}})^{\frac{1}{a_{nk}}}
% \end{align}

% We relax the Bernoulli distribution $q(z)$ to continuous using binary concrete distribution:
% \begin{align}
%     u &\sim \mathrm{Uniform}(0,1) \\
%     L &= \log (\frac{u}{1-u}) \\
%     z_{nk} &= \sigma(\frac{\text{logit}(\pi_{nk}) + L }{\text{temp}})
% \end{align}
% where $\text{logit}(\cdot)$ is inverse sigmoid function, temp is the relaxation temperature.

% \subsection{Inference} 
% The log likelihood of $p(A,X)$ can be computed by marginalizing over the latent variables defined in the generative process
% \begin{align}
%     p(A,X) = \int_{\mathcal{C}}\Big(\sum_{\mathcal{D}}p(A,X,\mathcal{C}, \mathcal{D})\Big)d\mathcal{C}
% \end{align}
% where $\mathcal{C} =\{C,W,\beta,\Theta,V\}$ are continuous variables  and  $\mathcal{D} =\{Z,Y\}$ are discrete variables, and 
% we have the joint probability $p(A,X,\mathcal{C}, \mathcal{D})=p(A,X,C,Z,W,\beta,\Theta,V,Y)$, which can be factorized as below:
% \begin{align}
%     &p(A,X,C,Z,W,\beta,\Theta,V,Y) \\
%     &= p(X|\beta,Y)p(Y|\Theta)p(A|Z,V)p(\beta)p(\Theta|Z,W) \\
%     &\cdot p(Z|C)p(C)p(W)p(V) 
% \end{align}
% We specify the posterior distribution $q_\phi(\cdot)$ as below, and factorize it into independent probabilities using mean-field theory:
% \begin{align}
%     &q_{\phi}(C,Z,W,\beta,\Theta,Y,V) \\
%     &= q_\phi(C)q_\phi(Z)q_\phi(W)q_\phi(\beta)q_\phi(\Theta) q_\phi(Y)q_\phi(V)
% \end{align}
% The variational distribution of latent variables are defined as below:
% \begin{align}
%     q(c_{nk}|a_{nk},b_{nk}) &= \mathrm{Beta}(a_{nk},b_{nk})\\
%     q(z_{nk}|\pi_{nk}) &= \mathrm{Bernoulli}(\pi_{nk})\\
%     q(w_{nk}|\gamma_{nk}) &= \mathrm{Gamma}(\gamma_{nk})\\
%     q(\beta_{kl}|\eta_{kl}) &= \mathrm{Dirichlet}(\eta_{kl})\\
%     q(\theta_{nk}|\psi_{nk}) &= \mathrm{Dirichlet}(\psi_{nk})\\
%     q(y_{nl}|\rho_{nl}) &= \mathrm{Discrete}(\rho_{nl})\\
%     q(v_{nk}|\mu_{nk}, \sigma_{nk}) &= \mathcal{N}(\mu_{nk}, \sigma_{nk})
% \end{align}
% The distribution parameters $\{a, b, \pi, \gamma, \eta, \psi,\rho, \mu, \sigma\}^N$ are parameterized by a neural network, which we will discuss later in section 4.2.
% \paragraph{Maximizing the ELBO}
% We need to maximize the variational lower bound $\mathcal{L}(\phi, A, X) \leq \log{p(A,X)}$:
% \begin{align}
%   &\mathcal{L}(\phi, A, X) \\&= \mathrm{E}_{q_\phi}\Big[\log{p(A,X,C,Z,W,\beta,\Theta,Y,V|B)} \\
%     &- \log{q_{\phi}(C,Z,W,\beta,\Theta,Y,V|A,X,B)}\Big]
% \end{align}
% The condition terms $A, X, B$ are omitted for simplicity.
% We further decompose the ELBO into:
% \begin{align*}
%   &\mathcal{L}(\phi, A, X) \\
%     &=\mathrm{E}_{q_{\phi}}\Big[\log{p(X|\beta,Y)} + \log{p(A|Z,V,B)}\Big] \\
%     &-\mathrm{KL}\big(q_{\phi}(\beta)||p(\beta)\big)- \mathrm{KL}\big(q_{\phi}(\Theta)||p(\Theta|Z,W)\big) \\ 
%     &-\mathrm{KL}\big(q_{\phi}(Z)||p(Z|C)\big) - \mathrm{KL}\big(q_{\phi}(C)||p(C)\big)\\
%     &-\mathrm{KL}\big(q_{\phi}(W)||p(W)\big) - \mathrm{KL}\big(q_{\phi}(V)||p(V)\big) \\
%     &-\mathrm{KL}\big(q_{\phi}(Y)||p(Y|\Theta)\big)
% \end{align*}
% which contains the likelihood of reconstructed edge and node, as well as the Kullback-Leibler(KL) divergence between the posterior and prior distributions of latent variables. 

% The reconstructed term of $X$ is calculated from every word feature in each document node:
% \begin{align}
%     \log{p(X|\beta,Y)} &=\sum_{n=1}^N\sum_{l=1}^{L_n}\log{p(x_{nl}|\beta_{y_{nl}})} 
% \end{align}
% where $x_{nl}$ is the $l$-th word occupancy in $n$-th document node, and $L_{n}$ denotes the counts of words in $n$-th document node.

% The reconstructed term of $A$ is from every pair of document nodes:
% \begin{align}
%     \log{p(A|Z,V,B)} = \sum_{n=1}^N\sum_{m=1}^N\log{p(A_{nm}|\sigma(r_n^TBr_m))}
% \end{align}
% where $r_n = v_n\odot z_n$, $\odot$ denotes the Hadamard product of two vectors in the same shape. The calculation of the KL terms are shown in the Appendix.

% \subsection{Variational Encoder}
% Here we show the design of the inference network, which approximate the true posterior distribution by outputting a set of parameters $\{a, b, \pi, \gamma, \eta, \psi,\rho, \mu, \sigma\}^N$ given input $A, X$. 
% we first show that the parameters $\{\pi,  \mu, \sigma\}^N$ are the output of Graph Convolutional Network (GCN) \cite{kipf2016semi}.
% \begin{align}
%   \{\pi,  \mu, \sigma\}^N = \mathrm{GCN}(A, X)
% \end{align}
% After we obtained these parameters, we can draw the membership vector $r_n=v_n\odot z_n$,
% where,
% \begin{align}
%     z_{nk}\sim q(z_{nk}|\pi_{nk});~v_{nk}\sim q(v_{nk}|\mu_{nk}, \sigma_{nk})
% \end{align}
% then we compute the parameters $\{\psi, \rho\}$ via a multi-head attention model (MHA) \cite{vaswani2017attention} utilizing the node feature $X$ and the sampled membership vector $R=\{r\}^N$. 
% \begin{align}
%     h_n = \mathrm{MLP}(x_n)\\
%     \{\psi, \rho\} = \mathrm{MHA}([r_n, h_n])
% \end{align}
% where $h_n$ is the sequence of word embeddings that belongs to the $n-th$ documents, in real application, node feature might be in the format of bag of words, which need to be converted into a corpus before feeding into the attention network. $r_n$ works as a [CLS] tokens, which capture the global context of the document, i.e. the topic distribution.

% To learn the latent structure information in the data, for each node $n$, we have $\pi,\gamma,\psi,\mu,\sigma$ learned from the GNN encoder with parameter $\phi$ as the weights in GNN.
% \begin{align}
%     \{\pi_{nk},\gamma_{nk},\psi_{nk},\mu_{nk},\sigma_{nk}\}_{n=1}^N = \mathrm{GNN}_{\phi}(A,X)
% \end{align}
% where we adopt GCN as the graph encoder. We use MLP encoder to learn parameters $a, b, \eta$ of variables $c, \beta$.

% % \paragraph{Self-attention Encoder}
% % We model the 
% % To better learn the topic information of the document node, we use self-attention layer as the encoder for $\rho$ of each node:

% % Turn multi-hot features x into sentence with word token: $X: [0,1,0,0,1,0...,1,1,0] -> D: [2, 5,...,1305, 1309, EOS]$.
% % Parameterize:$\theta$ for topic distribution $q(y|\rho)$ using self attention, each word has its own variational parameters.
% % For each document D: $\theta = \mathrm{self-attention}(D), \theta=\{\theta_1, …, \theta_L\}, D=\{d_1, … d_L\}$.
% %  Minimize reconstruction term: $E[-logP(D|Y,\beta)], Y\sim q(y|\theta), \beta\sim q(\beta|\eta)$
% % And minimize kl term:$KL(q(Y|\theta) || p(Y|z,w))$ and $KL(q(\beta|\eta)||p(\beta))$


% \subsection{Variational EM}
% In order to fit the block model $B$ along with the variational parameters, we seek to use Variational EM to iteratively train the model.

% In the E-step, we use Stochastic Gradient Variational Bayes (SGVB) to optimize the parameters of posterior of latent variables $C,Z,W,\beta,\Theta,V,Y$. Since back propagation can not be performed on non-differentiable latent variables, we employ the reparameterization tricks shown below.

% \paragraph{Reparameterization:} $v$ is sampled using reparameterization trick so that the Monte Carlo estimation of the normal distribution $q(v)$ is differentiable:
% \begin{align}
%     v_{nk} = \mu_{nk} + \sigma_{nk} \epsilon,\; \epsilon \sim \mathcal{N}(0, 1)
% \end{align}

% We approximate the Beta distribution $q(c)$ with Kumaraswamy distribution \cite{nalisnick2016stick}:
% \begin{align}
%     u &\sim \mathrm{Uniform}(0,1) \\
%     c_{nk} &= (1 - u^{\frac{1}{b_{nk}}})^{\frac{1}{a_{nk}}}
% \end{align}

% We relax the Bernoulli distribution $q(z)$ to continuous using binary concrete distribution \cite{maddison2016concrete}:
% \begin{align}
%     u &\sim \mathrm{Uniform}(0,1) \\
%     L &= \log (\frac{u}{1-u}) \\
%     z_{nk} &= \sigma(\frac{\text{logit}(\pi_{nk}) + L }{\text{temp}})
% \end{align}
% where $\text{logit}(\cdot)$ is inverse sigmoid function, temp is the relaxation temperature.

% We approximate the Dirichlet distribution $q(\beta)$ and $q(\theta)$ with Multi-Gamma distribution \cite{figurnov2018implicit}:
% \begin{gather}
%     \theta_{nk} \sim \mathrm{Gamma}(\psi_{nk},1) \\
%     \bigg(\frac{\theta_{n1}}{\sum_{k=1}^K \theta_{nk}} \cdots \frac{\theta_{nK}}{\sum_{k=1}^K \theta_{nk}}\bigg) \sim \mathrm{Dir}(\psi_{n1} \cdots \psi_{nK})
% \end{gather}

% We relax the Discrete distribution $q(y)$ to continuous using Gumbel-Softmax distribution \cite{jang2016categorical}:
% \begin{gather}
%     \lambda_l \sim \mathrm{Gumbel}(0,1) \;\;\;\; l=1, \cdots, L_n\\
%     y_{nl} = \frac{\text{exp}((\log(\rho_l) + \lambda_l)/\tau)}{\sum_{l=1}^{L_n}\text{exp}((\log(\rho_l) + \lambda_l)/\tau)} 
% \end{gather}

% For M-step, in the variational framework, the block model $B$ is treated as a hyperparameter and is fixed during E-step. To optimize $B$, we use the ELBO as the proxy of the log likelihood, and froze all the variational parameters. In ELBO, the only term that is related to $B$ is the edge reconstruction term, we define the loss function for optimizing $B$ as follow:
% \begin{align}
%     \mathcal{L}(B, \phi^*, A,X) = \mathrm{E}_{q_{\phi}}\Big[\log{p(A|Z,V,B)}\Big] +\lambda ||B||_1 
% \end{align}
% Since the non-activate entries in $B$ won't get training signal during the gradient descent, we add an L1 norm regularization term $||B||_1$ with coefficient $\lambda$, to push those entries to zero. $\phi^*$ denotes the fixed network parameters learned from the E-step. [TODO: add derivation to remove the expectation in this loss function]



% \section{Variational EM}

% \paragraph{Objective} We need to maximize the likelihood of recovered node $X$ and edge $A$ given the input training data:
% \begin{align}
%     & \log{p(\hat{A},\hat{X}|A,X)} \\
%     &\geq\mathrm{E}_{q}\Big[\log{p(\hat{A},\hat{X},C,Z,W,\beta,\Theta,Y,V|B)} \\
%     &- \log{q_{\phi}(C,Z,W,\beta,\Theta,Y,V|A,X,B)}\Big]
% \end{align}
% We specify the posterior distribution $q(\cdot)$ as below, and factorize it into independent probabilities using mean-field theory:
% \begin{align}
%     &q_{\phi}(C,Z,W,\beta,\Theta,Y,V) \\
%     &= q_\phi(C)q_\phi(Z)q_\phi(W)q_\phi(\beta)q_\phi(\Theta) q_\phi(Y)q_\phi(V)
% \end{align}
% the prior distribution $p(\cdot)$ can be factorized as follow based on the generative process:
% \begin{align}
%     &p(\hat{A},\hat{X},C,Z,W,\beta,\Theta,V,Y) \\
%     &= p(\hat{X}|\beta,Y)p(Y|\Theta)p(\hat{A}|Z,V)p(\beta)p(\Theta|Z,W) \\
%     & \cdot p(Z|C)p(C)p(W)p(V) 
% \end{align}
% The condition terms $A, X, B$ are omitted for simplicity.
% We further decompose the evidence lower bound (ELBO) into:
% \begin{align*}
%     &\mathcal{L}(C,Z,W,\beta,\Theta,V,Y) \\
%     &=\mathrm{E}_q\Big[\log{p(\hat{X}|\beta,Y)} + log{p(\hat{A}|Z,V,B)}\Big] \\
%     &-\mathrm{KL}\big(q(\beta)||p(\beta)\big)- \mathrm{KL}\big(q(\Theta)||p(\Theta|Z,W)\big) \\ 
%     &-\mathrm{KL}\big(q(Z)||p(Z|C)\big) - \mathrm{KL}\big(q(C)||p(C)\big)\\
%     &-\mathrm{KL}\big(q(W)||p(W)\big) - \mathrm{KL}\big(q(V)||p(V)\big) \\
%     &-\mathrm{KL}\big(q(Y)||p(Y|\Theta)\big)
% \end{align*}
% which contains the likelihood of reconstructed edge and node, as well as the Kullback-Leibler(KL) divergence between the posterior and prior distributions of latent variables. 
% The reconstructed node likelihood is calculated from every word feature in each document node:
% \begin{align}
%     \log{p(\hat{X}|\beta,Y)} &=\sum_{n=1}^N\sum_{l=1}^{L_n}\log{p(x_{nl}|\beta_{y_{nl}})} 
% \end{align}
% where $x_{nl}$ is the $l$-th word occupancy in $n$-th document node, and $L_{n}$ denotes the counts of words in $n$-th document node.
% The reconstructed edge likelihood is from every pair of document nodes:
% \begin{align}
%     \log{p(\hat{A}|Z,V,B)} = \sum_{n=1}^N\sum_{m=1}^N\log{p(\hat{A}_{nm}|\sigma(r_n^TBr_m))}
% \end{align}
% where $r_n = v_n\odot z_n$, $\odot$ denotes the Hadamard product of two vectors in the same shape.

% \subsection{Variational E-step}
% \paragraph{Posterior Inference} In the E-step of Variational EM, we use Stochastic Gradient Variational Bayes (SGVB) to optimize the parameters of posterior of latent variables $C,Z,W,\beta,\Theta,V,Y$.

% \paragraph{Reparameterization} $v$ is sampled using reparameterization trick so that the Monte Carlo estimation of the normal distribution $q(v)$ is differentiable:
% \begin{align}
%     v_{nk} = \mu_{nk} + \sigma_{nk} \epsilon,\; \epsilon \sim \mathcal{N}(0, 1)
% \end{align}

% We approximate the Beta distribution $q(c)$ with Kumaraswamy distribution:
% \begin{align}
%     u &\sim \mathrm{Uniform}(0,1) \\
%     c_{nk} &= (1 - u^{\frac{1}{b_{nk}}})^{\frac{1}{a_{nk}}}
% \end{align}

% We relax the Bernoulli distribution $q(z)$ to continuous using binary concrete distribution:
% \begin{align}
%     u &\sim \mathrm{Uniform}(0,1) \\
%     L &= \log (\frac{u}{1-u}) \\
%     z_{nk} &= \sigma(\frac{\text{logit}(\pi_{nk}) + L }{\text{temp}})
% \end{align}
% where $\text{logit}(\cdot)$ is inverse sigmoid function, temp is the relaxation temperature.

% We approximate the Dirichlet distribution $q(\beta)$ and $q(\theta)$ with Multi-Gamma distribution:
% \begin{gather}
%     \theta_{nk} \sim \mathrm{Gamma}(\psi_{nk},1) \\
%     \bigg(\frac{\theta_{n1}}{\sum_{k=1}^K \theta_{nk}} \cdots \frac{\theta_{nK}}{\sum_{k=1}^K \theta_{nk}}\bigg) \sim \mathrm{Dir}(\psi_{n1} \cdots \psi_{nK})
% \end{gather}

% We relax the Discrete distribution $q(y)$ to continuous using Gumbel-Softmax distribution:
% \begin{gather}
%     \lambda_l \sim \mathrm{Gumbel}(0,1) \;\;\;\; l=1, \cdots, L_n\\
%     y_{nl} = \frac{\text{exp}((\log(\rho_l) + \lambda_l)/\tau)}{\sum_{l=1}^{L_n}\text{exp}((\log(\rho_l) + \lambda_l)/\tau)} 
% \end{gather}

% \subsection{Variational M-step}
% \paragraph{Parameter Estimation} We use Stochastic Gradient Descent (SGD) to optimize block model $B$ to maximize ELBO given the approximated posterior of latent variables, which is the M-step of Variational EM.




==> tables/ablation_alpha.tex <==
% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{cccccc}
%     \hline
%         Alpha &1.0 & 1.5 & 2.0 & 2.5 & 3.0\\\hline 
%         \multicolumn{6}{c}{Cora}\\
%          20\% & 86.4 & 86.5 & 86.7 & 86.8 & 86.9\\
%          40\% & 90.7 & 90.8 & 90.9 & 91.1 & 91.4\\\hline
%         \multicolumn{6}{c}{Citeseer}\\
%         20\% & 92.2 & 92.6 & 92.8 & 92.9 & 93.1\\
%         40\% & 93.7 & 93.9 & 94.0 & 94.1 & 94.3\\
%         \hline
%     \end{tabular}
%     \label{tab:alpha}
%     \caption{Alpha sensitivity}
% \end{table}
% \begin{table}[t]
%     \centering
%     % \small
%     \begin{tabular}{ccccc}
%     \hline
%         \multirow{2}{*}{$\alpha$}&\multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Citeseer}\\
%         & 20\% & 40\% & 20\% & 40\%
%         \\
%         \hline 
%         % \multicolumn{5}{c}{Cora}\\
%          1.0 & 86.4 & 90.7 & 92.2 & 93.7\\
%          1.5 & 86.5 & 90.8 & 92.6 & 93.9\\
%          2.0 & 86.7 & 90.9 & 92.8 & 94.0\\
%          2.5 & 86.8 & 91.1 & 92.9 & 94.1\\
%          3.0 & 86.9 & 91.4 & 93.1 & 94.3\\\hline
         
%         % \multicolumn{5}{c}{Citeseer}\\\
%         % % w/ pbp
%         % 20\% & 88.5$\pm$0.76 & 92.2$\pm$0.55 & 93.6$\pm$0.59 & 94.5$\pm$0.12\\
%         % 40\% & 91.7$\pm$0.51 & 93.7$\pm$0.39 & 94.8$\pm$0.25 & 95.0$\pm$0.11\\
%         % 60\% & 92.8$\pm$0.58 & 94.5$\pm$0.42 & 95.5$\pm$0.30 & 95.5$\pm$0.31\\
%         % 80\% & 93.9$\pm$0.62 & 95.6$\pm$0.48 & 95.9$\pm$0.39 & 95.9$\pm$0.46\\
%         % \hline
%     \end{tabular}
%     \caption{Alpha sensitivity}
%     \label{ablation}
% \end{table}
\begin{table}[t]
    \centering
    \small
    \begin{tabular}{ccccccc}
    \hline
         \multirow{2}{*}{Dataset}&\multirow{2}{*}{Ratio}& \multicolumn{5}{c}{$\alpha$}\\
         &&1.0 & 1.5 & 2.0 & 2.5 & 3.0\\\hline 
        \multirow{2}{*}{Cora}&
        20\% & 86.4 & 86.5 & 86.7 & 86.8 & 86.9\\
         &40\% & 90.7 & 90.8 & 90.9 & 91.1 & 91.4\\\hline
        \multirow{2}{*}{Citeseer}&
        20\% & 92.2 & 92.6 & 92.8 & 92.9 & 93.1\\
        &40\% & 93.7 & 93.9 & 94.0 & 94.1 & 94.3\\
        \hline
    \end{tabular}
    \caption{Link prediction AUC increases on Cora and Citeseer with different training ratios as $\alpha$ gets larger.}
    \label{ablation_alpha}
\end{table}

==> tables/ablation_ratio.tex <==
% \begin{table}[t]
    \centering
    \scriptsize
    \begin{tabular}{ccccc}
    \hline
        \multirow{2}{*}{Ratio}&\multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Citeseer}\\
        & w/o ATN & w/ ATN & w/o ATN & w/ ATN 
        \\
        \hline 
        % \multicolumn{5}{c}{Cora}\\
         20\% & 82.7$\pm$0.61 & 86.4$\pm$0.58 & 88.5$\pm$0.76 & 92.2$\pm$0.55 \\
         40\% & 88.5$\pm$0.71 & 90.7$\pm$0.44 & 91.7$\pm$0.51 & 93.7$\pm$0.39\\
         60\% & 91.9$\pm$0.63 & 93.2$\pm$0.37 & 92.8$\pm$0.58 & 94.5$\pm$0.42\\
         80\% & 94.0$\pm$0.75 & 95.2$\pm$0.56 & 93.9$\pm$0.62 & 95.6$\pm$0.48\\\hline
        % \multicolumn{5}{c}{Citeseer}\\\
        % % w/ pbp
        % 20\% & 88.5$\pm$0.76 & 92.2$\pm$0.55 & 93.6$\pm$0.59 & 94.5$\pm$0.12\\
        % 40\% & 91.7$\pm$0.51 & 93.7$\pm$0.39 & 94.8$\pm$0.25 & 95.0$\pm$0.11\\
        % 60\% & 92.8$\pm$0.58 & 94.5$\pm$0.42 & 95.5$\pm$0.30 & 95.5$\pm$0.31\\
        % 80\% & 93.9$\pm$0.62 & 95.6$\pm$0.48 & 95.9$\pm$0.39 & 95.9$\pm$0.46\\
        % \hline
    \end{tabular}
    % \caption{The benefits of using attribute decoding at different sparsity levels: The percentage indicates the fraction of graph edges in the training set. The values are AUC values for link prediction. }
    % \label{tab:ablation_ratio}
% \end{table}



% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{ccccc}
%     \hline
%         \multirow{2}{*}{Ratio}&\multicolumn{2}{c}{NORAD} & \multicolumn{2}{c}{VGNAE}\\
%         & w/o ATN & w/ ATN & w/o ATN & w/ ATN 
%         \\
%         \hline 
%         \multicolumn{5}{c}{Cora}\\
%          20\% & 82.7$\pm$0.61 & 86.4$\pm$0.58 & 89.3$\pm$0.69 & 89.6$\pm$0.44\\
%          40\% & 88.5$\pm$0.71 & 90.7$\pm$0.44 & 92.1$\pm$0.34 & 92.2$\pm$0.34\\
%          60\% & 91.9$\pm$0.63 & 93.2$\pm$0.37 & 93.4$\pm$0.30 & 93.4$\pm$0.29\\
%          80\% & 94.0$\pm$0.75 & 95.2$\pm$0.56 & 94.6$\pm$0.24 & 94.6$\pm$0.30\\\hline
%         \multicolumn{5}{c}{Citeseer}\\\
%         % w/ pbp
%         20\% & 88.5$\pm$0.76 & 92.2$\pm$0.55 & 93.6$\pm$0.59 & 94.5$\pm$0.12\\
%         40\% & 91.7$\pm$0.51 & 93.7$\pm$0.39 & 94.8$\pm$0.25 & 95.0$\pm$0.11\\
%         60\% & 92.8$\pm$0.58 & 94.5$\pm$0.42 & 95.5$\pm$0.30 & 95.5$\pm$0.31\\
%         80\% & 93.9$\pm$0.62 & 95.6$\pm$0.48 & 95.9$\pm$0.39 & 95.9$\pm$0.46\\
%         \hline
%     \end{tabular}
%     \caption{Ablation Ratio}
%     \label{ablation}
% \end{table}



% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{ccccc}
%     \hline
%         \multirow{2}{*}{Ratio}&\multicolumn{2}{c}{NORAD} & \multicolumn{2}{c}{VGNAE}\\
%         & w/o ATN & w/ ATN & w/o ATN & w/ ATN 
%         \\\hline 
%         \multirow{5}{*}{Cora} & 20\% & 40\% & 60\% & 80\% \\
%          & 82.7$\pm$0.61 & 88.5$\pm$0.71 & 91.9$\pm$0.63 & 94.0$\pm$0.75\\
%          & 86.4$\pm$0.58 & 90.7$\pm$0.44 & 93.2$\pm$0.37 & 95.2$\pm$0.56\\
%          & 89.3$\pm$0.69 & 92.1$\pm$0.34 & 93.4$\pm$0.30 & 94.6$\pm$0.24\\
%          & 89.6$\pm$0.44 & 92.2$\pm$0.34 & 93.4$\pm$0.29 & 94.6$\pm$0.30\\\hline
%         \multirow{5}{*}{Citeseer} & 20\% & 40\% & 60\% & 80\% \\
%         % w/ pbp
%         & 88.5$\pm$0.76 & 91.7$\pm$0.51 & 92.8$\pm$0.58 & 93.9$\pm$0.62\\
%         & 92.2$\pm$0.55 & 93.7$\pm$0.39 & 94.5$\pm$0.42 & 95.6$\pm$0.48\\
%         & 93.6$\pm$0.59 & 94.8$\pm$0.25 & 95.5$\pm$0.30 & 95.9$\pm$0.39\\
%         & 94.5$\pm$0.12 & 95.0$\pm$0.11 & 95.5$\pm$0.31 & 95.9$\pm$0.46\\
%         \hline
%     \end{tabular}
%     \caption{Ablation Ratio}
%     \label{ablation}
% \end{table}



% \begin{table}[t]
%     \centering
%     \small
%     \begin{tabular}{ccccc}
%     \hline
%         ratio & base & norm & ATN & nATN\\\hline 
%         \multicolumn{5}{c}{Cora}\\
%          20\% & 82.7$\pm$0.61 & 86.2$\pm$1.15 & 86.4$\pm$0.58 & 87.9$\pm$0.49\\
%          40\% & 88.5$\pm$0.71 & 89.8$\pm$0.52 & 90.7$\pm$0.44 & 91.2$\pm$0.51\\
%          60\% & 91.9$\pm$0.63 & 91.8$\pm$0.61 & 93.2$\pm$0.37 & 92.6$\pm$0.71\\
%          80\% & 94.0$\pm$0.75 & 93.0$\pm$1.25 & 95.2$\pm$0.56 & 93.7$\pm$1.14\\\hline
%         \multicolumn{5}{c}{Citeseer}\\
%         20\% & 88.5$\pm$0.76 & 85.9$\pm$1.34 & 92.2$\pm$0.55 & 91.2$\pm$0.47\\
%         40\% & 91.7$\pm$0.51 & 90.1$\pm$1.04 & 93.7$\pm$0.39 & 93.3$\pm$0.72\\
%         60\% & 92.8$\pm$0.58 & 91.6$\pm$1.07 & 94.5$\pm$0.42 & 94.1$\pm$0.66\\
%         80\% & 93.9$\pm$0.62 & 92.8$\pm$1.09 & 95.6$\pm$0.48 & 94.8$\pm$0.70\\
%         \hline
%     \end{tabular}
%     \caption{Ablation Ratio}
%     \label{ablation}
% \end{table}

==> tables/algorithm.tex <==
\begin{algorithm}
\label{alg_EM}
  \caption{Varaitional EM for MTB}
  \label{alg:train}
  \begin{algorithmic}
    \STATE {\bfseries Input:} Dataset of graph $G = (X,A)$, 
    \STATE {\bfseries Output:} Learned node-wise representation $r$ and Blockmodel $B$
    \REPEAT   
        \STATE Initialize $(B, \theta, \phi)$
        \FOR{E step $= 1, \cdots $}
            \STATE Fix Blockmodel $B$
            \STATE Sample $r \sim q_{\phi}(r|X, A)$
            \STATE Optimize ($\phi, \theta$) by maximizing $\mathcal{L}(\phi, \theta, A, X|B)$
        \ENDFOR
        \FOR{M step $= 1, \cdots $}
            \STATE Fix parameters ($\phi, \theta$)
            \STATE Optimize $B$ by maximizing $\mathcal{L}(\phi, \theta, A, X|B)$
        \ENDFOR
    \UNTIL{convergence of the ELBO $\mathcal{L}(\phi, \theta, A, X|B)$}
  \end{algorithmic}
\end{algorithm}
